On the Effects of Heterogeneous Errors on Multi-fidelity Bayesian Optimization

Bayesian optimization (BO) is a sequential optimization strategy that is increasingly employed in a wide range of areas including materials design. In real world applications, acquiring high-fidelity (HF) data through physical experiments or HF simulations is the major cost component of BO. To alleviate this bottleneck, multi-fidelity (MF) methods are used to forgo the sole reliance on the expensive HF data and reduce the sampling costs by querying inexpensive low-fidelity (LF) sources whose data are correlated with HF samples. However, existing multi-fidelity BO (MFBO) methods operate under the following two assumptions that rarely hold in practical applications: (1) LF sources provide data that are well correlated with the HF data on a global scale, and (2) a single random process can model the noise in the fused data. These assumptions dramatically reduce the performance of MFBO when LF sources are only locally correlated with the HF source or when the noise variance varies across the data sources. In this paper, we dispense with these incorrect assumptions by proposing an MF emulation method that (1) learns a noise model for each data source, and (2) enables MFBO to leverage highly biased LF sources which are only locally correlated with the HF source. We illustrate the performance of our method through analytical examples and engineering problems on materials design.

==> Ref.tex <==
@article{shahriari2015taking,
  title={Taking the human out of the loop: A review of Bayesian optimization},
  author={Shahriari, Bobak and Swersky, Kevin and Wang, Ziyu and Adams, Ryan P and De Freitas, Nando},
  journal={Proceedings of the IEEE},
  volume={104},
  number={1},
  pages={148--175},
  year={2015},
  publisher={IEEE}
}

@article{frazier2018tutorial,
  title={A tutorial on Bayesian optimization},
  author={Frazier, Peter I},
  journal={arXiv preprint arXiv:1807.02811},
  year={2018}
}

@article{li2020multi,
  title={Multi-fidelity Bayesian optimization via deep neural networks},
  author={Li, Shibo and Xing, Wei and Kirby, Robert and Zhe, Shandian},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={8521--8531},
  year={2020}
}

@inproceedings{song2019general,
  title={A general framework for multi-fidelity bayesian optimization with gaussian processes},
  author={Song, Jialin and Chen, Yuxin and Yue, Yisong},
  booktitle={The 22nd International Conference on Artificial Intelligence and Statistics},
  pages={3158--3167},
  year={2019},
  organization={PMLR}
}

@inproceedings{takeno2020multi,
  title={Multi-fidelity Bayesian optimization with max-value entropy search and its parallelization},
  author={Takeno, Shion and Fukuoka, Hitoshi and Tsukada, Yuhki and Koyama, Toshiyuki and Shiga, Motoki and Takeuchi, Ichiro and Karasuyama, Masayuki},
  booktitle={International Conference on Machine Learning},
  pages={9334--9345},
  year={2020},
  organization={PMLR}
}
@inproceedings{zhang2019efficient,
  title={An efficient multi-fidelity bayesian optimization approach for analog circuit synthesis},
  author={Zhang, Shuhan and Lyu, Wenlong and Yang, Fan and Yan, Changhao and Zhou, Dian and Zeng, Xuan and Hu, Xiangdong},
  booktitle={Proceedings of the 56th Annual Design Automation Conference 2019},
  pages={1--6},
  year={2019}
}

@article{shu2021multi,
  title={A multi-fidelity Bayesian optimization approach based on the expected further improvement},
  author={Shu, Leshi and Jiang, Ping and Wang, Yan},
  journal={Structural and Multidisciplinary Optimization},
  volume={63},
  pages={1709--1719},
  year={2021},
  publisher={Springer}
}

@article{tran2020smf,
  title={sMF-BO-2CoGP: A sequential multi-fidelity constrained Bayesian optimization framework for design applications},
  author={Tran, Anh and Wildey, Tim and McCann, Scott},
  journal={Journal of Computing and Information Science in Engineering},
  volume={20},
  number={3},
  year={2020},
  publisher={American Society of Mechanical Engineers Digital Collection}
}

@article{xiao2018extended,
  title={Extended Co-Kriging interpolation method based on multi-fidelity data},
  author={Xiao, Manyu and Zhang, Guohua and Breitkopf, Piotr and Villon, Pierre and Zhang, Weihong},
  journal={Applied Mathematics and Computation},
  volume={323},
  pages={120--131},
  year={2018},
  publisher={Elsevier}
}

@article{kennedy2001bayesian,
  title={Bayesian calibration of computer models},
  author={Kennedy, Marc C and O'Hagan, Anthony},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={63},
  number={3},
  pages={425--464},
  year={2001},
  publisher={Wiley Online Library}
}

@article{gardner2018gpytorch,
  title={Gpytorch: Blackbox matrix-matrix gaussian process inference with gpu acceleration},
  author={Gardner, Jacob and Pleiss, Geoff and Weinberger, Kilian Q and Bindel, David and Wilson, Andrew G},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@article{foumani2023multi,
  title={Multi-fidelity cost-aware Bayesian optimization},
  author={Foumani, Zahra Zanjani and Shishehbor, Mehdi and Yousefpour, Amin and Bostanabad, Ramin},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={407},
  pages={115937},
  year={2023},
  publisher={Elsevier}
}

@inproceedings{escamilla2003hybrid,
  title={Hybrid Kalman filter-fuzzy logic adaptive multisensor data fusion architectures},
  author={Escamilla-Ambrosio, P Jorge and Mort, Neil},
  booktitle={42nd IEEE International Conference on Decision and Control (IEEE Cat. No. 03CH37475)},
  volume={5},
  pages={5215--5220},
  year={2003},
  organization={IEEE}
}

@article{kreibich2013quality,
  title={Quality-based multiple-sensor fusion in an industrial wireless sensor network for MCM},
  author={Kreibich, Ondrej and Neuzil, Jan and Smid, Radislav},
  journal={IEEE Transactions on Industrial Electronics},
  volume={61},
  number={9},
  pages={4903--4911},
  year={2013},
  publisher={IEEE}
}

@article{eweis2022data,
  title={Data Fusion With Latent Map Gaussian Processes},
  author={Eweis-Labolle, Jonathan Tammer and Oune, Nicholas and Bostanabad, Ramin},
  journal={Journal of Mechanical Design},
  volume={144},
  number={9},
  pages={091703},
  year={2022},
  publisher={American Society of Mechanical Engineers}
}

@article{oune2021latent,
  title={Latent map Gaussian processes for mixed variable metamodeling},
  author={Oune, Nicholas and Bostanabad, Ramin},
  journal={Computer Methods in Applied Mechanics and Engineering},
  volume={387},
  pages={114128},
  year={2021},
  publisher={Elsevier}
}

@article{bostanabad2018leveraging,
  title={Leveraging the nugget parameter for efficient Gaussian process modeling},
  author={Bostanabad, Ramin and Kearney, Tucker and Tao, Siyu and Apley, Daniel W and Chen, Wei},
  journal={International journal for numerical methods in engineering},
  volume={114},
  number={5},
  pages={501--516},
  year={2018},
  publisher={Wiley Online Library}
}

@article{carvalho2010horseshoe,
  title={The horseshoe estimator for sparse signals},
  author={Carvalho, Carlos M and Polson, Nicholas G and Scott, James G},
  journal={Biometrika},
  volume={97},
  number={2},
  pages={465--480},
  year={2010},
  publisher={Oxford University Press}
}

@article{gal2014distributed,
  title={Distributed variational inference in sparse Gaussian process regression and latent variable models},
  author={Gal, Yarin and Van Der Wilk, Mark and Rasmussen, Carl Edward},
  journal={Advances in neural information processing systems},
  volume={27},
  year={2014}
}
@inproceedings{mohammed2017over,
  title={Over-fitting in model selection with Gaussian process regression},
  author={Mohammed, Rekar O and Cawley, Gavin C},
  booktitle={Machine Learning and Data Mining in Pattern Recognition: 13th International Conference, MLDM 2017, New York, NY, USA, July 15-20, 2017, Proceedings 13},
  pages={192--205},
  year={2017},
  organization={Springer}
}

@article{lindley1982scoring,
  title={Scoring rules and the inevitability of probability},
  author={Lindley, Dennis V},
  journal={International Statistical Review/Revue Internationale de Statistique},
  pages={1--11},
  year={1982},
  publisher={JSTOR}
}

% @article{winkler1996scoring,
%   title={Scoring rules and the evaluation of probabilities},
%   author={Winkler, Robert L and Munoz, Javier and Cervera, Jos\'{e} L and Bernardo, Jos\'{e} M and Blattenberger, Gail and Kadane, Joseph B and Lindley, Dennis V and Murphy, Allan H and Oliver, Robert M and R\'{\i}os-Insua, David},
%   journal={Test},
%   volume={5},
%   pages={1--60},
%   year={1996},
%   publisher={Springer}
% }

@article{scoring_rules,
  title={Strictly proper scoring rules, prediction, and estimation},
  author={Gneiting, Tilmann and Raftery, Adrian E},
  journal={Journal of the American statistical Association},
  volume={102},
  number={477},
  pages={359--378},
  year={2007},
  publisher={Taylor \& Francis}
}

@article{bracher2021evaluating,
  title={Evaluating epidemic forecasts in an interval format},
  author={Bracher, Johannes and Ray, Evan L and Gneiting, Tilmann and Reich, Nicholas G},
  journal={PLoS computational biology},
  volume={17},
  number={2},
  pages={e1008618},
  year={2021},
  publisher={Public Library of Science San Francisco, CA USA}
}

@article{mitchell2017proper,
  title={Proper scoring rules for interval probabilistic forecasts},
  author={Mitchell, K and Ferro, CAT},
  journal={Quarterly Journal of the Royal Meteorological Society},
  volume={143},
  number={704},
  pages={1597--1607},
  year={2017},
  publisher={Wiley Online Library}
}

@article{gneiting2007strictly,
  title={Strictly proper scoring rules, prediction, and estimation},
  author={Gneiting, Tilmann and Raftery, Adrian E},
  journal={Journal of the American statistical Association},
  volume={102},
  number={477},
  pages={359--378},
  year={2007},
  publisher={Taylor \& Francis}
}

@article{mora2023probabilistic,
  title={Probabilistic Neural Data Fusion for Learning from an Arbitrary Number of Multi-fidelity Data Sets},
  author={Mora, Carlos and Eweis-Labolle, Jonathan Tammer and Johnson, Tyler and Gadde, Likith and Bostanabad, Ramin},
  journal={arXiv preprint arXiv:2301.13271},
  year={2023}
}

@article{yeom2019performance,
  title={Performance evaluation of automobile fuel consumption using a fuzzy-based granular model with coverage and specificity},
  author={Yeom, Chan-Uk and Kwak, Keun-Chang},
  journal={Symmetry},
  volume={11},
  number={12},
  pages={1480},
  year={2019},
  publisher={MDPI}
}

@article{herbol2018efficient,
  title={Efficient search of compositional space for hybrid organic--inorganic perovskites via Bayesian optimization},
  author={Herbol, Henry C and Hu, Weici and Frazier, Peter and Clancy, Paulette and Poloczek, Matthias},
  journal={npj Computational Materials},
  volume={4},
  number={1},
  pages={51},
  year={2018},
  publisher={Nature Publishing Group UK London}
}
